DRAGON: Drone and Ground Gaussian Splatting for 3D Building Reconstruction

3D building reconstruction from imaging data is an important task for many applications ranging from urban planning to reconnaissance. Modern Novel View synthesis (NVS) methods like NeRF and Gaussian Splatting offer powerful techniques for developing 3D models from natural 2D imagery in an unsupervised fashion. These algorithms generally require input training views surrounding the scene of interest, which, in the case of large buildings, is typically not available across all camera elevations. In particular, the most readily available camera viewpoints at scale across most buildings are at near-ground (e.g., with mobile phones) and aerial (drones) elevations. However, due to the significant difference in viewpoint between drone and ground image sets, camera registration - a necessary step for NVS algorithms - fails. In this work we propose a method, DRAGON, that can take drone and ground building imagery as input and produce a 3D NVS model. The key insight of DRAGON is that intermediate elevation imagery may be extrapolated by an NVS algorithm itself in an iterative procedure with perceptual regularization, thereby bridging the visual feature gap between the two elevations and enabling registration. We compiled a semi-synthetic dataset of 9 large building scenes using Google Earth Studio, and quantitatively and qualitatively demonstrate that DRAGON can generate compelling renderings on this dataset compared to baseline strategies.

==> algorithms/dragon_weights.tex <==
\begin{algorithm}[t!]
\caption{\bsname{} fixed$(\text{model}, X_\text{train}, C_\text{train}, C_\text{test},\alpha)$}
\begin{algorithmic}[1]
\Statex Given NVS model, train images $X_\text{train}$, 
\Statex train camera poses $C_\text{train}$, test camera poses $C_\text{test}$
% \Statex elevation $E = \{E_\text{ground}, E_1, \dots E_N, E_\text{drone} \}$
% \State \textcolor{gray}{\% Perform registration to obtain camera poses}
% \State $C_\text{train} = \text{COLMAP}(X_\text{train})$
\State $\text{model.train}(X_\text{train}, C_\text{train}, \alpha)$ 
\State $X_{\text{test}} = \text{model.test}(C_\text{test})$ 
\State $\textbf{return } X_\text{test}$
\end{algorithmic}
\label{alg:basic_weights}
\end{algorithm}


\begin{algorithm}[t!]
\caption{Dragon fixed$(\text{model}, X_\text{train},N,\alpha)$}
\begin{algorithmic}[1]
\Statex Given NVS model, $X_\text{train} = X^{0} \cup X^{N}$,
\Statex number of elevation levels $N$
\Statex weighting scheme $\alpha$ (image-wise and elevation-wise)
\Statex (potentially "learn" $\alpha$)
\State $X_\text{test} = \emptyset$
\State $X^\text{cum} = X^N$
\For{$i = N-1$ to $1$} \textcolor{gray}{\% iterate over elevations}
    % \State $X^\text{cum} = X^\text{cum} \cup X^{i}$
    \State $C^\text{cum} = \text{COLMAP}(X^\text{cum})$
    \State $X^{i-1} = \text{BASIC}(\text{model}, X^\text{cum}, C^\text{cum}, C^{i-1}, \alpha)$
    \State $X^\text{cum} = X^\text{cum} \cup X^{i-1}$
    \State $X_\text{test} = X_\text{test} \cup X^{i-1}$
\EndFor
\State $X^\text{cum} = X^\text{cum} \cup X^{0}$
\State $C_\text{cum} = \text{COLMAP}(X^\text{cum})$
\State $\textbf{return }X_\text{test} \cup   \text{BASIC}(\text{model}, X_\text{cup}, C_\text{cum}, C_\text{test}, \alpha)$
\end{algorithmic}
\label{alg:dragon_weights}
\end{algorithm}

==> figures_tex/clip_heatmap.tex <==
\begin{figure}
\includegraphics[width=0.5\textwidth]{figures/eiffel_heatmap.png}
\caption{Clip heatmap}
\label{fig:eiffel_heatmap}
\end{figure}

==> figures_tex/colmap_struggle.tex <==
\begin{figure}[t!]
\centering
\includegraphics[width=0.49\textwidth]{figures/matching_results22.pdf}
\caption{Left: Basic registers on average only 50\%  of the ground truth images. Right: Dragon registers correctly over 97\% of ground images while also having significantly lower registration errors. \mm{aesthetics will be improved}}
\label{fig:colmap_struggle}
\end{figure}

==> figures_tex/eiffel_rebuttal.tex <==
\begin{figure}[h]
\centering
\includegraphics[width=\linewidth]{figures/eiffel.png}
\caption{\textbf{Higher-level images (left)
offer a more comprehensive view of the building than ground-level (right) ones.}}
\label{fig:eiffel}
\end{figure}

==> figures_tex/final_render_b3.tex <==
\begin{figure*}[t!]
\centering
\includegraphics[width=0.9\textwidth]{figures/paris_qualitative.pdf}
\caption{final rendering: Arc de Triomphe. Qualitative comparison between Basic (drone) and Dragon}
\label{fig:result-rendering-b3}
\end{figure*}

==> figures_tex/reg_basic.tex <==
\begin{figure}[t!]
\centering
\includegraphics[width=0.49\textwidth]{figures/registration_basic.pdf}
\caption{Basic registration pipeline}
\label{fig:reg_ours}
\end{figure}

==> tables/tab_buildings_radius.tex <==
\begin{table*}[t]
    \caption{\textbf{Camera radii and target altitudes per elevation for each building in \dsname{}, our proposed dataset.} We set these values manually per building by \gb{yujin, fill in}. \gb{Can we combine these numbers with the Table 1? These numbers don't seem very important to be in their own table.}}
    \resizebox{\linewidth}{!}{
        \begin{tabular}{|C{2.5cm}|*{9}{C{1.7cm}|}}
        \hline
           {\diagbox[width=2.5cm]{Elevation}{Building}} &   Arc de Triomphe & Colosseum & Duomo di Milano & Eiffel Tower & Himeji Castle & Piazza del Duomo & Space Needle  & Sydney Opera House & The Gateway Arch \\
            \hline
Ground & 250m / 89m & 313m / 52m & 250m / 153m & 438m / 89m & 250m / 67m & 250m / 34m & 188m / 71m & 438m / 48m & 313m / 166m \\
Mid 1  & 313m / 89m & 375m / 52m & 438m / 152m & 500m / 89m & 313m / 67m & 250m / 34m & 250m / 71m & 438m / 48m & 375m / 166m \\
Mid 2  & 375m / 89m & 438m / 52m & 500m / 177m & 625m / 114m & 375m / 67m & 313m / 34m & 250m / 95m & 563m / 48m & 438m / 203m \\
Mid 3  & 500m / 89m & 500m / 52m & 438m / 152m & 750m / 151m & 375m / 67m & 313m / 34m & 375m / 120m & 563m / 48m & 563m / 203m \\
Drone  & 313m / 89m & 500m / 52m & 375m / 152m & 375m / 177m & 313m / 67m & 313m / 34m & 313m / 145m & 500m / 48m & 375m / 203m \\
\hline
        \end{tabular}
    }
    \label{tab:scenes_radius}
\end{table*}

% backup radius/altitude/target
% Ground & 250/101/89 & 313/77/52 & 250/177/153 & 438/101/89 & 250/92/67 & 250/58/34 & 188/83/71 & 438/60/48 & 313/166/166 \\
% Mid 1  & 313/201/89 & 375/127/52 & 438/250/152 & 500/201/89 & 313/154/67 & 250/146/34 & 250/195/71 & 438/148/48 & 375/240/166 \\
% Mid 2  & 375/301/89 & 438/252/52 & 500/402/177 & 625/351/114 & 375/279/67 & 313/246/34 & 250/345/95 & 563/298/48 & 438/403/203 \\
% Mid 3  & 500/451/89 & 500/452/52 & 438/600/152 & 750/601/151 & 375/404/67 & 313/346/34 & 375/495/120 & 563/498/48 & 563/603/203 \\
% Drone  & 313/701/89 & 500/702/52 & 375/802/152 & 375/1000/177 & 313/604/67&313/596/34 & 313/695/145 & 500/748/48 & 375/803/203 \\

==> tables/tab_oracle1.tex <==
\begin{table}[H]
\centering
\caption{PSNR for oracle methods. oracle-0,1,2 is BASIC trained on both images and camera poses from elevations 0,1,2 and evaluated on all elevations.}
\label{table:oracle1}
\begin{tabular}{|c|*{6}{c|}}
\hline
method                & elev 0 (ground) & elev 1 & elev 2 & elev 3 & elev 4 (drone) \\
\hline
$\text{oracle-0}$     & 0               & 0      & 0      & 0      & 0     \\         
$\text{oracle-0,1}$     & 0      & 0     & 0     & 0     & 0     \\            
$\text{oracle-0,1,2}$     & 0      & 0     & 0     & 0     & 0     \\            
$\text{oracle-0,1,2,3}$     & 0      & 0     & 0     & 0     & 0     \\            
$\text{oracle-0,1,2,3,4}$     & 0      & 0     & 0     & 0     & 0     \\            
$\text{oracle-0,4}$   & 0               & 0      & 0      & 0      & 0     \\    
$\text{oracle-4}$     & 0      & 0     & 0     & 0     & 0     \\            
\hline
\end{tabular}
\end{table}


==> tables/tab_oracle_cpnoise.tex <==
\begin{table}[H]
\centering
\caption{oracle method with added CP noise. oracle-0,1*,2** *(0,0.1), **(0.1, 0.3) means we added (0 mean 0.1 std) noise to first elevation, and (0.1 mean 0.3 std) to second elevation  }
\label{table:oracle2}
\begin{tabular}{|c|*{7}{c|}}
\hline
method                & noise & elev 0 (ground) & elev 1 & elev 2 & elev 3 & elev 4 (drone) \\
\hline
$\text{oracle-0,1*,2**}$ & *(0,0.1), **(0.1, 0.3)       & 0               & 0      & 0      & 0      & 0     \\         
\hline
\end{tabular}
\end{table}


==> tables/tab_oracle_exclude.tex <==
\begin{table}[H]
\centering
\caption{oracle method with excluded images.oracle-0,1*,2**; *(5\%), **(20\%) means 5\% images were excluded from 1st elevation and 20\% images were excluded from 2nd elevation }
\label{table:oracle3}
\begin{tabular}{|c|*{7}{c|}}
\hline
method                & excluded & elev 0 (ground) & elev 1 & elev 2 & elev 3 & elev 4 (drone) \\
\hline
$\text{oracle-0,1*,2**}$ & *(5\%), **(20\%)       & 0               & 0      & 0      & 0      & 0     \\         
\hline
\end{tabular}
\end{table}


==> tables/tab_psnr_ablation.tex <==
\begin{table*}
\caption{\mm{this will be modified. im leaving it for reference}}
\label{table:metrics3}
{\tiny
\begin{tabular}{llllllllllllllll}
\hline\noalign{\smallskip}
& \multicolumn{3}{l}{drone} & \multicolumn{3}{l}{mid 1} & \multicolumn{3}{l}{mid 2} & \multicolumn{3}{l}{mid 3} & \multicolumn{3}{l}{ground} \\
\noalign{\smallskip}
\hline
& PSNR$\uparrow$ & SSIM$\uparrow$ & LPIPS$\downarrow$ & PSNR$\uparrow$ & SSIM$\uparrow$ & LPIPS$\downarrow$ & PSNR$\uparrow$ & SSIM$\uparrow$ & LPIPS$\downarrow$ & PSNR$\uparrow$ & SSIM$\uparrow$ & LPIPS$\downarrow$ & PSNR$\uparrow$ & SSIM$\uparrow$ & LPIPS$\downarrow$ \\
\noalign{\smallskip}
\hline
%              % ------ drone ------ % ------ mid 1 ------ % ------ mid 2 ------ % ------ mid 3 ------ % ------ ground ------ 
%              % PSNR  % SSIM % LPIP % PSNR  % SSIM % LPIP % PSNR  % SSIM % LPIP % PSNR  % SSIM % LPIP % PSNR  % SSIM % LPIP 
BASIC          & 27.63 & 0.90 & 0.14 & 21.30 & 0.73 & 0.29 & 17.77 & 0.57 & 0.41 & 13.98 & 0.41 & 0.55 & 7.46 & 0.28 & 0.60 \\
Dragon         & 26.90 & 0.88 & 0.14 & 20.57 & 0.68 & 0.34 & 16.34 & 0.54 & 0.50 & 15.46 & 0.50 & 0.47 & 25.11 & 0.84 & 0.18 \\
Dragon w/o DreamSim & 26.87 & 0.88 & 0.14 & 20.28 & 0.67 & 0.34 & 17.17 & 0.55 & 0.48 & 13.24 & 0.40 & 0.64 & 25.36 & 0.85 & 0.17 \\
\end{tabular}
}
\end{table*}

\begin{table*}
\centering
\caption{\textbf{Quantitative comparison of our method.} We report SSIM, PSNR and LPIPS on test views at 5 different elevations (drone, ground, and 3 intermediate levels). The best and second-best results are highlighted. This is the average score, and the score for each building is in the supplement. The dataset consists of 10 different buildings in various locations. \mm{i will modify this table and I will add barplots}}
\label{table:metrics}
\begin{tabular}{m{2cm}|*{3}{c|}*{3}{c|}*{3}{c|}}
 &\multicolumn{3}{c|}{ground and drone} &\multicolumn{3}{c|}{mid elevations} &\multicolumn{3}{c|}{all elevations} \\ \hline
 & PSNR$\uparrow$ & SSIM$\uparrow$ & LPIPS$\downarrow$ & PSNR$\uparrow$ & SSIM$\uparrow$ & LPIPS$\downarrow$ & PSNR$\uparrow$ & SSIM$\uparrow$ & LPIPS$\downarrow$ \\
\hline
%              % -- drone and ground - % -- mid elevations --  %  -- all elevations -- 
%              % PSNR  % SSIM  % LPIPS % PSNR  % SSIM  % LPIPS % PSNR  % SSIM  % LPIPS  
BASIC          & 17.54          & 0.59           & 0.37           & \textbf{17.68} & \textbf{0.57}  & \textbf{0.42}  
& 17.63          & 0.58          & 0.40  \\
Dragon         & 26.01          & \textbf{0.86}  & \textbf{0.16}  & 17.46          & \textbf{0.57}  & 0.44 
& \textbf{20.88} & \textbf{0.69}  & \textbf{0.33}  \\
Dragon w/o DreamSim & \textbf{26.12} & \textbf{0.86}  & \textbf{0.16}  & 16.90          & 0.54           & 0.49  
& 20.58          & 0.67           & 0.35  \\
\end{tabular}
\end{table*}

%              % -- drone and ground - % -- mid elevations --  %  -- all elevations -- 
%              % PSNR  % SSIM  % LPIPS % PSNR  % SSIM  % LPIPS % PSNR  % SSIM  % LPIPS  
% BASIC          & 17.54 & 0.59  & 0.37  & 17.68 & 0.57  & 0.42  & 17.63 & 0.58  & 0.40  \\
% Dragon-vanilla & 26.11 & 0.86  & 0.16  & 16.90 & 0.54  & 0.49  & 20.58 & 0.67  & 0.35  \\
% Dragon         & 26.01 & 0.86  & 0.16  & 17.46 & 0.57  & 0.44 & 20.87 & 0.69  & 0.33  \\









% \end{center}
% \setlength{\tabcolsep}{1.4pt}

% Drone-only     & 27.63&0.90&0.14 & 21.30&0.73&0.29 & 17.77&0.57&0.41 & 13.98&0.41&0.55 & 7.46&0.28&0.60\\
% Ground-only     & 9.42&0.25&0.65 & 9.46&0.27&0.64 & 9.93&0.32&0.61 & 12.27&0.41&0.53 & 26.36&0.86&0.16\\

==> tables/tab_supp_eiffel.tex <==
% \begin{table*}[h]
% \caption{\textbf{Registration performance comparison.} Eiffel tower}
% \label{table:spsg}
% \centering
% \begin{tabular}{|cc|c|c|c|c|c|}
% \hline
% \multicolumn{2}{|c}{} & \multicolumn{2}{|c}{1-HEADED} & \multicolumn{3}{|c|}{2-HEADED} \\ \cline{3-7}
% \multicolumn{2}{|c}{} & \multicolumn{1}{|c|}{COLMAP} & \multicolumn{1}{c|}{COLMAP} & \multicolumn{1}{c|}{COLMAP} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}DRAGON\\ vanilla\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}DRAGON\\ DreamSim\end{tabular}} \\ \cline{3-7}
% \multicolumn{2}{|c}{} & \multicolumn{1}{|c|}{drone-only} & \multicolumn{1}{c|}{ground-only} & \multicolumn{3}{c|}{drone\&ground} \\ \hline
% \multicolumn{2}{|c|}{Matched (\%) $\uparrow$}  & 100.00 & 79.58 & 50.00 & 88.00 & \textbf{97.47} \\ \hline
% \multicolumn{1}{|c|}{Errors for matched} & rotation ($^{\circ}$) $\downarrow$ & 0.76/0.68 & 19.13/2.39 & 0.69/0.60 & 0.15/0.12 & \textbf{0.12/0.10} \\ \cline{2-2}
% \multicolumn{1}{|c|}{(Avg/Std)} & position (m) $\downarrow$ & 0.02/0.02 & 0.50/0.05 & 0.02/0.02 & 0.02/0.02 & \textbf{0.01/0.01} \\ \hline
% \end{tabular}
% \end{table*}

\begin{table}[]
\caption{\textbf{Registration performance comparison.} Eiffel tower}
\label{table:spsg-eiffel}
\resizebox{\textwidth}{!}{%
\begin{tabular}{|cc|c|c|}
\hline
\multicolumn{2}{|c|}{}                              & COLMAP & SPSG \\ \hline
\multicolumn{2}{|c|}{Matched (\%) $\uparrow$}       &  50.00   &  50.00  \\ \hline
\multicolumn{1}{|c|}{Errors for matched} & rotation ($^{\circ}$) $\downarrow$ &  0.31/0.08   &  0.53/0.09    \\ \cline{2-4} 
\multicolumn{1}{|c|}{(Avg/Std)}          & position (m) $\downarrow$ &   0.01/0.01     &  0.03/0.02    \\ \hline
\end{tabular}%
}
\end{table}
